Frontier Language Models are not Robust to Adversarial Arithmetic, or "What do I need to say so you agree 2+2=5?

We introduce and study the problem of adversarial arithmetic, which provides a simple yet challenging testbed for language model alignment. This problem is comprised of arithmetic questions posed in natural language, with an arbitrary adversarial string inserted before the question is complete. Even in the simple setting of 1-digit addition problems, it is easy to find adversarial prompts that make all tested models (including PaLM2, GPT4, Claude2) misbehave, and even to steer models to a particular wrong answer. We additionally provide a simple algorithm for finding successful attacks by querying those same models, which we name "prompt inversion rejection sampling" (PIRS). We finally show that models can be partially hardened against these attacks via reinforcement learning and via agentic constitutional loops. However, we were not able to make a language model fully robust against adversarial arithmetic attacks.

==> main_old.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}
% \usepackage{listings}
% \usepackage[most]{tcolorbox}

% \title{Adversarial Arithmetic}
% \author{cdfreeman, laculp, aarontp, mlbileschi, gamaleldin, addmorepeopleeee }
% \date{August 2023}

% \usepackage{natbib}
% \usepackage{graphicx}

% \begin{document}

% \maketitle
% \abstract{Hello this is an abstract.}

% \section{Introduction}

% Large transformer-based models exhibit a rich variety of behaviors, spanning superhuman performance on manifold natural language and reasoning tasks, to surprising failures of capability and unreliability of execution on other, often related, tasks.

% As the capability frontier of large models expands, it becomes ever more pressing to better understand and control the boundary of these capability failures.  Various techniques have emerged as scalable flywheels for exerting fine control of models.  In particular, the combination of RL(H/AI)F and automated red-teaming has proved fruitful in allowing practitioners to sculpt the behavior of large models by leveraging models to generate and curate high quality datasets, and to bootstrap off of powerful learned reward models for circumscribing high dimensional, natural-language notions of ``reward''.

% While these techniques have greatly improved the quality of models, particularly in sculpting behaviors towards better interactive assistants and instruction-following machines, there remain significant gaps in both characterizing and hardening the frontier of model failures.

% Fully characterizing this frontier is difficult.  While we want models to be ``aligned''---fully specifying what that even means at best requires an overwhelming additional complexity in the form of added epicycles---special casing, localisation, deferment to human overseers, etc.,---and at worst reduces to a task as hard as fully specifying human morality, which is not even uniquely defined amongst humans.

% Thus, we reduce our scope to the problem of arithmetic questions posed in natural language.  We ask, ``Can frontier models be aligned to do arithmetic, even in the presence of adversaries that may try to steer them astray?''.

% This formulation neatly sidesteps the problem of having to perfectly specify a complicated or even controversial notion of ``alignment'' by simply requiring that a model answer arithmetic questions correctly---though making this judgment is still sometimes not as straightforward as it might seem.  This problem likewise inherits the breadth and complexity of natural language, providing a rich attack surface where an ``aligned'' model needs to be robust.  That is to say, it's a problem for which verification of ``good behavior'' is easy, but fully enumerating all of the vectors of attack is a similar kind of difficult as the more general problem of alignment.

% As a summary of our results, we provide:
% \begin{itemize}
%     \item A simple algorithm for generating semantically rich adversarial attacks that transfer across model families, and which reliably steer non-hardened models to make arithmetic errors. \ref{sec:pirs}
%     \item Scaling results for model resistance to attack after hardening as a function of dataset size, model size, and dataset variety.
%     \item Evaluation results cataloging model performance change during training, including on out-of-distribution model attacks.
%     \item Characterizations of mitigation effectiveness for debate loops, constitutional loops, and additional rounds of hardening.
%     \item Additionally, we release a dataset of prompts and model continuations/attacks that may be of independent interest.
% \end{itemize}

% Ultimately, we find that it is possible to greatly suppress the tendency of frontier models to assert false arithmetic statements in this adversarial setting, but that we still cannot fully remove this ``vulnerability''.

% % The remainder of the paper is organized as follows.

% % In Sec. \ref{sec:problem}, we lay out the

% % blah

% % blah

% % cite cite cite

% \subsection{Prior art in large model attacks}

% cite cite cite cite

% \section{Problem Setup}

% We consider an adversarial training procedure where a Red model, $R$, seeks attacks, $x \in D$, that steer a Blue model, $B$, to satisfy some target badness criteria, $L(x)$ via some search procedure $S$.  One ``round'' of adversarial training proceeds in 2 steps.

% \begin{enumerate}
%     \item $R$ generates a dataset $D$ of attacks according to a search procedure $S$.
%     \item $B$ is trained to minimize $L(x)$ over the dataset.
% \end{enumerate}

% In principle, these steps need not be strictly serial, but in our experiments, they are.  There exist various interesting choices and prior art for these components.  Where relevant, we indicate which models were used for $R$ and $B$, we use PPO to train our models (see Appendix PPO Details for more information), and we use the technique outlined in \ref{sec:pirs} to search for attacks comprising $D$.



% \section{Adversarial Generation}

% Many techniques have been pioneered for eliciting specific ``dangerous'' continuations from models, like jailbreaking, soft-prompt tuning, and even directly optimizing tokens.  While gradient-based methods with white-box model access typically result in more powerful attacks, the attacks themselves are also typically somewhat inscrutable, reminiscent of the noisy-looking adversarial vulnerabilities that have plagued image-based models for years.  While these classes of attacks are obviously important, and have critical alignment ramifications, we instead focus on more semantically understandable attacks---i.e., attacks that make sense in natural language---as they can be indicative of more egregious reasoning failures.

% \subsection{Prompt Inversion Rejection Sampling}

% With the exception of hand-authored out of distribution attacks mentioned in Sec. LATERSECTION, all of the attacks in this work were generated via an algorithm we call Prompt Inversion Rejection Sampling.

% Intuitively, we would like to be able to invert the process $p(x=\rm{bad} | y)$ to find those tokens $y$ that result in particular ``bad'' $x$'s.  Large models are not invertible, so this is usually hard.  However, sufficiently large models can sometimes be used to directly perform this inversion via a prompt with the schematic form:

% \begin{tcolorbox}[colback=red!20!white, colframe=gray!75!black]
% ``X, therefore \{something bad\}.

% What is the value of X? \{additional constaints on X\}.

% X:"
% \end{tcolorbox}

% For arithmetic problems, we use such a template to have the model generate arguments that would make it answer arithmetic problems incorrectly.  For example:

% \begin{tcolorbox}[colback=red!20!white, colframe=gray!75!black]
% ``Provide the solution to the following arithmetic problem.


% \{x\} + \{y\} = Z


% ARGUMENT

% Thus, \{x\} + \{y\} = \{x+y+w\}.

% What is the value of ARGUMENT?  ARGUMENT should use a significant amount of creativity, drawing on various sources of science, mathematics, literature, and logic.  It can invoke a chain of thought, be an argument, or even be lyrical in its content.  Avoid the phrase 'the answer is' in any of your responses.

% ARGUMENT:"
% \end{tcolorbox}

% Such a prompt provides a way to generate candidate attacks by instructing the model to generate an argument for why it would say, e.g., that ``2 + 2 = 5''.  One need only have an additional evaluation prompt to determine if the attack was successful.  Again, in arithmetic, we use:

% \begin{tcolorbox}[colback=blue!20!white, colframe=gray!75!black]
% ``Provide the solution to the following arithmetic problem.

% \{x\} + \{y\} = Z


% \{attack\}

% Thus, \{x\} + \{y\} ="
% \end{tcolorbox}

% Evaluation simply checks to see whether the blue model is successfully steered to answer the arithmetic question wrong.

% Thus, prompt inversion rejection sampling proceeds as follows:

% \begin{enumerate}
%     \item Using Red model, sample candidate prompt inversions using the attack prompt.
%     \item Using Blue model, evaluate candidate attacks with the eval prompt.  If attack succeeds, accept, otherwise, reject and go back to step 1.
% \end{enumerate}



% % description of method with an example prompt

% \subsection{Attack Success Probability}
% % e.g., scaling with number of digits and wrongness and temperature
% % also probability of successful generation as a function of model size of generating model

% In this section, we examine the likelihood of the attack succeeding as a function of various attack and model properties.

% We consider several different attack prompts, catalogued in Appendix APPENDIXGOHERE.  Each of these prompts can be used to generate attacks that are parametric with respect to the amount ``wrong'' that the attack is trying to steer the model.  For example, $2+2=5$ has ``wrongness=1''.  For the attacks in this section, we consider 1-digit arithmetic with wrongness randomly sampled between 1 and 10.  Each attack was sampled independently and randomly for adding two numbers between 1 and 10.  Fig. \ref{fig:attack_succes_v_size} depicts the scaling of attack likelihood with model size over 1,000 independent attacks, for several different attack families.  The overall trend is noisy, but indicates weak inverse-scaling, where the attack effectiveness \emph{increases} with model size, though this trend is not strict, and varies with each attack.

% Fig. \ref{fig:attack_success_v_wrongness} indicates the scaling of attack success probability with amount of ``wrongness'' in the attack.  Here, trends are even noisier, though it is typically the case that attack success \emph{increases} with amount of wrongness.  Additionally, we monitor ``steerable'' wrongness, which is the likelihood any given attack steered a model towards a particular wrong answer, specified in the attack.  We note that the probability of successfully steering a model to a particular wrong answer is (by definition) upper bounded by the probability of the attack succeeding, and it's usually not much below this upper bound.  Note that this bound is sometimes saturated---i.e., every attack that succeeded also successfully steered the model to the target wrong answer, as in, e.g., the ``chain\_of\_thought'' attack.
% \begin{figure*}[h]
% \includegraphics[width=\linewidth]{figures/attack_success_v_size.pdf}
% \caption{TODO: add error bars, add final datapoint. Probability of attack success as a function of model size (billions of parameters) for several different attack types.  Prompts used for attack generation available in Appendix APPENDIXGOHERE.  Attacks were generated using a 340 billion parameter instruction-tuned model. \label{fig:attack_succes_v_size}}
% \end{figure*}

% \begin{figure*}[h]
% \includegraphics[width=\linewidth]{figures/attack_success_v_wrongness.pdf}
% \caption{TODO: add error bars, add final datapoints. Probability of attack success as a function of attack ``wrongness''---i.e., the amount by which the attack is trying to steer the model to make an incorrect answer.  Prompts used for attack generation available in Appendix APPENDIXGOHERE.  In each subpane, different colors indicate different model sizes.  Solid cirlces indicate attack success probability, and crosses indicated ``steered'' success probability---i.e., whether the attack successfully steered a model to make a particular wrong answer.  Attacks were generated using a 340 billion parameter instruction-tuned model. \label{fig:attack_success_v_wrongness}}
% \end{figure*}

% % TODO: Attack success probability on a 24B model as a function of different generators (1b 8b 24b 340b???)

% \subsection{Attack Transfer Success}
% % not sure how much we can say here, perhaps a chatgpt experiment?

% \section{Adversarial Hardening}

% \subsection{Hyperparameter Optimization}

% \subsection{Model Size Scaling}

% \subsection{Dataset Size Scaling}

% \subsection{True Negative Scaling}

% % e.g., wrongness-percentage experiments


% \section{Evaluation Metrics}

% \subsection{Sequence Copying}

% \subsection{Random Templating}

% \subsection{Procedural Word Problems}

% \subsection{Out of Distribution Attacks}

% \subsubsection{Context Overwhelming}

% \subsubsection{Authoritative Tool}

% \subsubsection{Long Confusing Algebra}

% \subsubsection{Suffix Variation} % i.e., Laura's various suffix modifications

% % tool misspecification
% % context overflow
% % long-algebra

% \subsubsection{Multilingual attacks}

% \subsection{In Distribution Failures}
% % e.g., stubborn negatives / examples that still work even after training

% \subsection{Auxiliary Tasks}

% % e.g., bigbench bleu/rouge scores during training.

% \section{Multi-round Hardening}

% % stretch goal --- how stuff changes as attack generation / hardening procedure is run multiple times

% \section{Agentic Mitigations and Attacks}

% \subsection{Constitutional Loops}

% % TODO

% \subsection{Constitutional Attacks}

% % stretch

% \section{Discussion and Outlook}

% \section{Broader Impacts}

% \appendix {Training Details} % ppo training details
% \appendix {Datasets and Prompts} % dataset and prompt inversion templates
% \appendix {Additional Plots} % every single plot imaginable


% \bibliographystyle{plain}
% \bibliography{references}
% \end{document}

